Reflections on trusting distributed trust

Many systems today distribute trust across multiple parties such that the system provides certain security properties if a subset of the parties are honest. In the past few years, we have seen an explosion of academic and industrial cryptographic systems built on distributed trust, including secure multi-party computation applications (e.g., private analytics, secure learning, and private key recovery) and blockchains. These systems have great potential for improving security and privacy, but face a significant hurdle on the path to deployment. We initiate study of the following problem: a single organization is, by definition, a single party, and so how can a single organization build a distributed-trust system where corruptions are independent? We instead consider an alternative formulation of the problem: rather than ensuring that a distributed-trust system is set up correctly by design, what if instead, users can audit a distributed-trust deployment? We propose a framework that enables a developer to efficiently and cheaply set up any distributed-trust system in a publicly auditable way. To do this, we identify two application-independent building blocks that we can use to bootstrap arbitrary distributed-trust applications: secure hardware and an append-only log. We show how to leverage existing implementations of these building blocks to deploy distributed-trust systems, and we give recommendations for infrastructure changes that would make it easier to deploy distributed-trust systems in the future.

==> Makefile <==
ms.pdf: FORCE
	latexmk -pdf -pvc -latexoption=-halt-on-error \
		-latexoption=-file-line-error \
		-latexoption=-interaction=nonstopmode \
		-latexoption=-synctex=1 ms.tex \
		&& touch ms.dvi 
.PHONY: FORCE

.PHONY: evince clean
evince:
	evince ms.pdf &

clean:
	latexmk -pdf -C ms


==> fonts.tex <==

\usepackage[T1]{fontenc}
\usepackage{newtxmath}
\usepackage{newtxtext}

% Use slightly smaller-than-default \texttt
\usepackage[scaled=.8]{beramono}

% Use normal mathcal
\DeclareMathAlphabet\mathcal{OMS}{cmsy}{m}{n}
\SetMathAlphabet\mathcal{bold}{OMS}{cmsy}{b}{n}

% Use normal mathsf
\SetMathAlphabet{\mathsf}{normal}{OT1}{cmss}{m}{n}
\SetMathAlphabet{\mathsf}{bold}{OT1}{cmss}{bx}{n}

% Use AMS mathbb
\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareSymbolFontAlphabet{\mathbb}{AMSb}


% Use times for numbers
\DeclareSymbolFont{numbers}{T1}{ptm}{m}{n}
\SetSymbolFont{numbers}{bold}{T1}{ptm}{bx}{n}
\DeclareMathSymbol{0}\mathalpha{numbers}{"30}
\DeclareMathSymbol{1}\mathalpha{numbers}{"31}
\DeclareMathSymbol{2}\mathalpha{numbers}{"32}
\DeclareMathSymbol{3}\mathalpha{numbers}{"33}
\DeclareMathSymbol{4}\mathalpha{numbers}{"34}
\DeclareMathSymbol{5}\mathalpha{numbers}{"35}
\DeclareMathSymbol{6}\mathalpha{numbers}{"36}
\DeclareMathSymbol{7}\mathalpha{numbers}{"37}
\DeclareMathSymbol{8}\mathalpha{numbers}{"38}
\DeclareMathSymbol{9}\mathalpha{numbers}{"39}

% Use times for operators
\SetSymbolFont{numbers}{bold}{T1}{ptm}{b}{n}
\makeatletter
\renewcommand{\operator@font}{\mathgroup\symnumbers}
\makeatother

% 10pt on 11pt
\makeatletter
\iffalse
\renewcommand\normalsize{%
   \@setfontsize\normalsize{10pt}{11.55pt}%
   \abovedisplayskip 11\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}

\renewcommand\small{%
  \@setfontsize\small{9pt}{2pt}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\makeatother
\fi



==> relatedwork.tex <==
\section{Related Work}
\begin{itemize}
    \item Code Verify~\cite{code-verify}
    \begin{itemize}
        \item Web extension that verifies the version of WhatsApp user is running on their browser
        \item WhatsApp server uploads hash of code for a given version to cloudflare -- cannot modify hash for that version once it's set
        \item Web extension computes hash on library served by WhatsApp and compares to hash held by Cloudflare
    \end{itemize}
    \item Subsource Integrity
    \begin{itemize}
        \item Add integrity tag to asset on html page; protects against malicious CDN (assuming the html page is not tampered with)
    \end{itemize}
    \item Binary Transparency~\cite{binary-transparency}
    \begin{itemize}
        \item Uses a tamper-evident append-only log (Trillian) to store hash of code at every release
        \item User checks their downloaded code against the log before executing
    \end{itemize}
\end{itemize}
